Exact Imposition of Safety Boundary Conditions in Neural Reachable Tubes

Hamilton-Jacobi (HJ) reachability analysis is a widely adopted verification tool to provide safety and performance guarantees for autonomous systems. However, it involves solving a partial differential equation (PDE) to compute a safety value function, whose computational and memory complexity scales exponentially with the state dimension, making its direct application to large-scale systems intractable. To overcome these challenges, DeepReach, a recently proposed learning-based approach, approximates high-dimensional reachable tubes using neural networks (NNs). While shown to be effective, the accuracy of the learned solution decreases with system complexity. One of the reasons for this degradation is a soft imposition of safety constraints during the learning process, which corresponds to the boundary conditions of the PDE, resulting in inaccurate value functions. In this work, we propose ExactBC, a variant of DeepReach that imposes safety constraints exactly during the learning process by restructuring the overall value function as a weighted sum of the boundary condition and the NN output. Moreover, the proposed variant no longer needs a boundary loss term during the training process, thus eliminating the need to balance different loss terms. We demonstrate the efficacy of the proposed approach in significantly improving the accuracy of the learned value function for four challenging reachability tasks: a rimless wheel system with state resets, collision avoidance in a cluttered environment, autonomous rocket landing, and multi-aircraft collision avoidance.

==> intro_Somil.tex <==
\section{Introduction}
With the recent surge in real-world applications of autonomous systems, ensuring the safety of these systems is becoming increasingly important. One effective approach to formalize the safety of autonomous systems is via Hamilton-Jacobi (HJ) Reachability analysis \cite{8263977}. In HJ reachability analysis, a Backward Reachable Tube (BRT) of the system is computed. The BRT is the set of all initial states of the system from which it can be driven to a target set within a specified time horizon, despite the worst-case disturbance (e.g., modeling error, environment disturbance, or an adversarial agent). Therefore, the BRT comprises the assuredly safe states under the optimal safe controller for the system. Conversely, the target set can also represent the desirable set of states, whose corresponding BRT identifies unsafe states for the system and should be avoided. Along with the BRT, the reachability analysis also yields a safe controller for the system to maintain system safety.

HJ reachability analysis frames the BRT computation as an optimal control problem. This eventually results in solving a partial differential equation (PDE), called Hamilton-Jacobi-Isaacs (HJI) PDE, over the state space to obtain the value function corresponding to this optimal control problem. Once computed, the sub-zero level set of the value function yields the BRT. Traditionally, this PDE is solved numerically over a state-space grid \cite{mitchell2005time,lygeros2004reachability,fisac2015reach,liao2024improved}. However, the computational complexity of grid-based methods scales exponentially with the number of state dimensions, limiting their direct application to systems up to 5D.

Several recent advancements have been made to mitigate this ``curse of dimensionality.'' Some approaches impose assumptions on system dynamics, such as linearity \cite{darbon2016algorithms,chow2017algorithm,lee2020hopf} or monotonicity \cite{coogan2015efficient}, to compute the value function for high-dimensional systems. Alternative methods decompose system dynamics to reduce a high-dimensional reachability problem to several smaller subproblems \cite{chen2015exact,10365682}. However, these methods do not offer a general framework for handling high-dimensional system dynamics within HJ reachability analysis. To overcome these challenges, learning-based methods have been proposed to compute neural approximations of the reachable tubes and the value function \cite{9561949, darbon2020overcoming, niarchos2006neural,djeridane2006neural,rubiesroyo2017recursive,jiang2016using}. 

Among these, a promising class of methods leverages deep neural networks to approximate the safety value function, such as DeepReach \cite{9561949}. DeepReach leverages advances in implicit neural representations \cite{sitzman2020} and physics-informed neural networks \cite{raissi2019physics} to solve the HJI PDE. Specifically, the safety value function is represented as a neural network whose weights are optimized by using a combination of two loss terms -- (a) the residual errors arising from enforcing the boundary conditions of the HJI PDE, which corresponds to the specification of the target set (also referred to as the \textit{safety specification} from here on) and (b) the residual errors associated with the HJI PDE within the domain’s interior. A notable advantage of DeepReach is that, unlike grid-based methods, its complexity doesn’t scale exponentially with the system dimensions, thereby allowing it to handle high-dimensional reachability problems. Nevertheless, the accuracy of the learned solution suffers from the ability to co-optimize the two loss terms and the relative weight between them. Additionally, the imposition of the safety specifications as a soft constraint makes it particularly prone to learning inaccurate value functions, as the solution of any PDE depends heavily on the boundary conditions. This drawback is more acute for complex boundary conditions (e.g., cluttered obstacles for a mobile robot), where DeepReach may learn completely non-physical solutions.

In this work, we take inspiration from earlier efforts in physics-informed machine learning models \cite{saad2022guiding, li2020fourier,li2021physics，sukumar2022exact} to overcome the aforementioned challenges by proposing a new variant of DeepReach that exactly satisfies the safety constraints (i.e., the boundary conditions). Rather than using the neural network (NN) to learn the value function directly, our key idea, aligned with the work of \cite{lagaris1998artificial}, is to represent the value function as a weighted combination of the boundary value function and the neural network output, where the NN output is weighted by a ``distance function'' to the boundary. This distance function is zero at the boundary and increases as the system state is farther from the boundary. Consequently, we show that the learned value function always satisfies the boundary conditions. 
Corresponding to this novel formulation, we derive a new loss function to train the neural network.
Since the network needs to optimize only a single loss function, which corresponds to the HJI PDE residual errors, it eliminates the scope of inaccuracies that could stem from the incorrect weighting of two loss terms. 
Overall, we show that the proposed method significantly enhances the accuracy of the learned safety value function.
To summarize, our overall contributions are:
\begin{enumerate}
    \item We propose a new method to increase the accuracy of deep learning-based approximation of high-dimensional reachable tubes.
    \item Our proposed variant computes the value function by optimizing a single loss function, thereby eliminating the need for hyperparameter tuning and the scope of inaccuracies that could stem from the incorrect weighting of two loss terms.
    \item We illustrate the benefits of the proposed strategy through case studies on two high-dimensional reachability problems: a 6D Rocket Landing problem and a 9D three-vehicle collision avoidance problem, both of which are intractable for traditional methods.
\end{enumerate}

==> related_work.tex <==
\section{Related work}
\subsection{BRT Computation via HJ Reachability}
\label{sec:HJ_rw}
Several methods have been proposed to compute BRT using Hamilton-Jacobi reachability analysis.
% HJ Reachability literature
% HJ Reachability analysis is a powerful tool to provide formal safety assurances and synthesize safe controllers for dynamical systems. Since it is grounded in dynamic programming, it suffers from the curse of dimensionality. 
%
Traditionally, level-set methods \cite{mitchell2005time,lygeros2004reachability,fisac2015reach,liao2024improved} compute BRTs by solving an HJI partial differential equation (PDE) on a discretized grid of the state-space. However, the computational complexity of these methods scales exponentially with the system dimensionality, which limits a direct application of these methods to systems up to 5D. 

%
\cite{8263977} provides a comprehensive survey of various methods that have been introduced to reduce the aforementioned computation burden.
%
For example, several works impose assumptions on the system dynamics to compute the value function for high-dimensional systems, such as linearity \cite{darbon2016algorithms,chow2017algorithm,lee2020hopf} or monotonicity \cite{coogan2015efficient}. %
%
Alternative methods decompose system dynamics to reduce a high-dimensional reachability problem to several smaller subproblems \cite{chen2015exact,10365682}.
% manipulate the system dynamics by decomposition or linearization to learn an approximate value function and \cite{herbert2019reachability} warm-starts value function computation with the aid of certain initialization. 
However, none of the above approaches offer a framework to handle general high-dimensional system dynamics within HJ reachability analysis.
To overcome these challenges, learning-based methods have been proposed to compute neural approximations of the reachable tubes and the value function \cite{9561949, darbon2020overcoming, niarchos2006neural,djeridane2006neural,rubiesroyo2017recursive,jiang2016using}.
% and PDE solvers are on the rise for this task as they don't compute the BRTs numerically, which makes them compatible with high-dimensional reachability problems. \cite{darbon2020overcoming} use a Shallow Neural Network, and \cite{niarchos2006neural,djeridane2006neural,royo2016recursive,jiang2016using} use Deep Neural Networks (DNN) to compute the value function. 
As a special realization of neural PDE solvers, DeepReach \cite{9561949} took advantage of the periodic (sinusoidal) activation function to accurately learn the safety value function and demonstrated its success on high-dimensional reachability problems. 
However, the learned solution is prone to errors as DeepReach imposes boundary conditions as soft constraints during the training process. 
Additionally, DeepReach requires the user to carefully choose the hyperparameter balancing the imposition of boundary constraints and the PDE constraints, which can affect the learned solution quality.
% its two loss terms in training, PDE loss from the interior of the domain and boundary loss from the boundaries of the domain, which becomes non-trivial when the boundary condition is complex. 
This work builds upon DeepReach and aims to overcome these limitations by imposing the boundary conditions exactly during the learning process. 
% by doing away with these limitations. 
% Our method optimizes a single loss function to learn the value function and imposes exact boundary conditions to enhance the accuracy of the earned HJ reachability solution.  

% PINN literature
\subsection{Imposing Exact Boundary Condition in Physics Informed Machine Learning Models}
%
In general, a PDE can have infinitely many solutions, and boundary conditions are defined to recover a particular solution of the PDE. 
% Hence, boundary conditions hold crucial physical meaning and are the sole signal that anchors the overall solution of PDEs for boundary value problems (BVPs).
%
Hence, an inexact boundary value function can lead to inaccurate or even non-physical solutions. In addition, training with a composition of boundary loss and PDE loss compromises the convergence of the stochastic gradient descent algorithm \cite{sukumar2022exact,wang2020understanding,chen2020comparison}.
%

To address these challenges, some recent works have studied the imposition of exact boundary conditions with neural ODE and PDE solvers.
%
\cite{saad2022guiding, li2020fourier,li2021physics} modified the structure of kernels within neural operators to make the model always satisfy boundary conditions. 
% Nonetheless, this method requires the learned solution to be expressed as an integral operator with the kernel, i.e., the base approximator falls in the class of neural operators such as \cite{li2020fourier,li2021physics} which is not compatible with DeepReach.
%
\cite{sukumar2022exact} proposes a method for imposing boundary constraints for physics-informed neural networks (PINNs) by constructing an approximate distance function to the boundary. 
%
% For dirichlet boundary condition the solution structure is $V=g+\phi \tilde{V}$, where $\tilde{V}$ is a neural network approximation, g is the boundary function, and V is the solution of PDE. 
%
However, constructing a complex distance function is generally time-consuming and unnecessary for imposing boundary conditions in the HJI PDE. 
%
In one of the earlier studies, \cite{lagaris1998artificial} represented the trial solution of PDE by the sum of two terms. The first term is a fixed function satisfying the boundary conditions, and the second term is the product of the neural network approximation and a function that zeroes out at the boundary of the domain. 
%
% While this insight is not well extended to high-dimensional and more general BVPs in the PINN domain because of the existence of irregular boundary conditions, it is well suited for HJ reachability problems where the boundary condition is merely time boundary constraints.
%
Our work takes inspiration from this idea and presents a more specific formulation that caters to the HJI PDE. We also propose a pretraining scheme to facilitate learning stability under the new solution structure.
% \zfnote{Should we test more models, such as l(x)+NN(x,t)-NN(x,0), to distinct ourselves from this idea?}
